An Analysis of DES Cluster Simulations through the IMCAT and Shapelets Weak Lensing Pipelines

We have run two completely independent weak lensing analysis pipelines on a set of realistic simulated images of a massive galaxy cluster with a singular isothermal sphere profile (galaxy velocity dispersion sigma_v=1250 km/ sec). The suite of images was constructed using the simulation tools developed by the Dark Energy Survey. We find that both weak lensing pipelines can accurately recover the velocity dispersion of our simulated clusters, suggesting that current weak lensing tools are accurate enough for measuring the shear profile of massive clusters in upcoming large photometric surveys. We also demonstrate how choices of some cuts influence the final shear profile and sigma_v measurement. Analogously to the STEP program, we make all of these cluster simulation images publically available for other groups to analyze through their own weak lensing pipelines.

==> secs/mntests.tex <==
\section{PSF Removal Test}
\label{sec:tests}

In order to test how well we are removing the PSF, we implemented a
test which we refer to as a `stars on stars' test, by which we mean a
check where we correct half of the stars (randomly selected throughout
the field) for PSF distortion in an image, by the PSF interpolated
from the other half of the stars throughout the field.  In general,
the size of the corrected stars in such a test should become smaller
and the ellipticities of these stars should shrink substantially.

Because a linear variation in \ellipy\ and FWHM of the stars was put
into the PSF, we expect that a linear order \interpln\ of the PSF will
be sufficient to adequately describe the PSF across the field.  This
is indeed what we find; numerically, after a linear order PSF
correction, taking the 200-300 stars per CCD on the files and dividing
them into two pieces, we find for the average and width of the values
of the \ellips\ of the PSF-corrected stars the values in
Table~\ref{table:ellips}. These results indicate a reduction by
between one and two orders of \mag\ in the \avg\ of each component of
the \ellipy, and a reduction by about a third in the \ellipy\ width
distribution.


\begin{table}
 \centering
  \caption{Table of \avg\ stellar \ellips\ and their widths before and after PSF-removal stars on stars test (see \secref{sec:tests}).}
 \label{table:ellips}
  \begin{tabular}{@{}|l|l|l|l|l| @{}}
  \hline
  \hline
 File & \eone\ \Avg\ & \etwo\ \Avg\ & $\sigma_{\eone}$  & $\sigma_{\etwo}$  \\
\hline
\hline
Before PSF removal &  -0.0132 & -0.0110 &  0.0121 &  0.0112 \\
\hline
After PSF removal &  0.0008  &  0.0009  & 0.0095  &  0.0082 \\
\hline
\hline
\end{tabular}
\end{table}

We also did this at several other orders -- at zero'th order (constant
stellar \ellipy\ and FWHM assumed across whole plane), we found that
in fact the \avg\ \ellips\ were of the same order as before
correction, and the widths barely shifted.  And above order one, there
was no significant reduction in either the \avg\ \ellips\ nor widths
above that already gained by the order one PSF removal, all indicating
that a order one \interpln\ is sufficient to describe the PSF variation
across the CCD.


